Efficient and Near-Optimal Smoothed Online Learning for Generalized Linear Functions

Due to the drastic gap in complexity between sequential and batch statistical learning, recent work has studied a smoothed sequential learning setting, where Nature is constrained to select contexts with density bounded by 1/{\sigma} with respect to a known measure {\mu}. Unfortunately, for some function classes, there is an exponential gap between the statistically optimal regret and that which can be achieved efficiently. In this paper, we give a computationally efficient algorithm that is the first to enjoy the statistically optimal log(T/{\sigma}) regret for realizable K-wise linear classification. We extend our results to settings where the true classifier is linear in an over-parameterized polynomial featurization of the contexts, as well as to a realizable piecewise-regression setting assuming access to an appropriate ERM oracle. Somewhat surprisingly, standard disagreement-based analyses are insufficient to achieve regret logarithmic in 1/{\sigma}. Instead, we develop a novel characterization of the geometry of the disagreement region induced by generalized linear classifiers. Along the way, we develop numerous technical tools of independent interest, including a general anti-concentration bound for the determinant of certain matrix averages.

==> body/checklist.tex <==
%!TEX root = ../neurips_submission.tex

\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{Our claimed contributions are efficiently achievable regret bounds for certain function classes in the smoothed online learning setting.  Right before the related work section, we have a paragraph describing the structure and pointing to where each of the claims is discussed.}
  \item Did you describe the limitations of your work?
    \answerYes{Note that we are only claiming results for particular function classes in the smoothed online learning setting (see contributions).}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{See the statements of each proposition and lemma, along with the relevant preliminaries as needed.}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{All proofs are included in the appendix.}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNA{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerNA{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNA{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerNA{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}

==> body/noisy_alg.tex <==
%!TEX root = ../smoothonlineoptimistic.tex
\newpage
\newcommand{\labell}{\mathsf{label}}
\newcommand{\labeled}{\mathsf{prelab}}
\newcommand{\Fepoch}{\cF^{\mathrm{epoch}}}
\newcommand{\epsep}{\epsilon_{\mathrm{sep}}}
\newcommand{\Delsep}{\mathsf{\Delta}_{\mathrm{sep}}}
\newcommand{\N}{\mathbb{N}}
\section{Algorithms with Noise}

\subsection{Classification}
We consider 
\begin{itemize}
	\item Algorithm proceeds in epochs $s$ of length $\tau_s$
	\item For each epoch $s$, we have a lower bound $N_s$ on the size of a minimal ``good'' cluster (something in terms of MSE and separation). 
	\item We define the set of all clusters $C_s$ of size $\ge N_s$ at epoch $s$ as $\scrC_s$. 
	\item We define a ``probabilistic label'' as follows:
	\begin{align*}
	\forall C \in \scrC_s,  \labell(C) = \begin{cases} \labell(C_{s'}) & \text{ for any } C' \in \scrC_{s'} \text{ s.t. } \|\fhat_{C_{s,C}} - \fhat_{s',C'}\|_{\square} \le \epsep. \\
	\text{'something new'} & \text{otherwise} \\
	\end{cases}
	\end{align*} 
	We call the $C \in \scrC_s$ in the former case ``pre-labeled'', and call the set of such $C$'s $\labeled(\scrC_s)$. 
\end{itemize}

\begin{lemma} For all epochs $s$, there exist some $\pi_s$ such that, for all $s' \le s$, for all $C' \in \scrC_{s'}$
\begin{align*}
\{\#  z \in C': \pi_s(\labell(C')) \ne g_{\star}(z) \} \le \mathrm{ErrTerm} \approx \tilde{O}(\sqrt{\frac{1}{\Delsep|C'|}})
\end{align*}
\end{lemma}

\begin{lemma} Fix an epoch $s$. Given $s+1$,
\begin{align*}
\forall C \in \labeled(\scrC_{s+1}), \E[ | \Fepoch_s ]
\end{align*}
\end{lemma}
\newcommand{\pihat}{\hat{\pi}}
\newcommand{\ghat}{\hat{g}}
\newcommand{\gst}{g^{\star}}
\newcommand{\fst}{f^{\star}}

\newcommand{\I}{\mathbb{I}}
\subsection{Classification to Regression}
At each time $t$, fix an ERM, get $\fhat_{t,1},\dots,\fhat_{t,k}$. Then you devise a permutation $\pihat_t$ which ``aligns'' $\fhat_{t,i}$ ith labeled clusters. Then for new $x_t$, you predict $\ghat_t(x_t)$ from classifier. Then, you predice $\fhat_{t,\pihat_t(\ghat_t(x))}$. 

\begin{align*}
(\fhat_{t,\pihat_t(\ghat_t(x))} - \fst)^2 \le B^2 \I\{\pihat_t(\ghat_t(x)) \ne \gst(x) \} + (\fhat_{t,\pihat_t(\ghat)})
\end{align*}

\newpage

\section{More Formally}
\newcommand{\ErrTerm}{\mathrm{Err}}
\newcommand{\Mistake}{\mathrm{Mist}}
\begin{definition}[Error] We say a function $\ErrTerm(\cdot,\cdot): \N \times (0,1) \to \reals_{\ge 0}$ is an \emph{valid error term} if, with probability $1-\delta$, for all $s$ and all $C \in \scrC_s$,
\begin{align*}
\exists i \text{s.t. } \|\fst_i - \fhat_{C}\|_{2}^2 \le \ErrTerm(|C|,\delta). 
\end{align*}
\end{definition}

\begin{lemma} For a gamelength $T$ and minimal length $N_s$,  $\ErrTerm(N,\delta) \le \dots$ is a valid error term. 
\end{lemma}

\newcommand{\labst}{\mathsf{label}_{\star}}
\mscomment{fuck with constants}
\begin{lemma}\label{lem:true_assignment_noisy} Suppose that $\ErrTerm(N_s,\delta) < \Delsep^2/16$. Then, for every $s,s'$ and everu $C \in \scrC_{s}$, there exists
\begin{itemize}
\item Exactly one $i$ such that $\|\fst_i - \fhat_{C}\|_{2} < \Delsep/4$. We call this $\labst(C)$. 
\item at most one $C' \in \scrC_{s'}$ such that $\|\fhat_{C} - \fhat_{C'}\| < \Delsep/2$. 
\item If $\labst(C') = \labst(C)$, then $\|\fhat_{C} - \fhat_{C'}\| < \Delsep/2$.
\end{itemize} 

\end{lemma}

\begin{lemma}[Correctness of the Labeling Operator]
\end{lemma}
\begin{proof}
As a consequence of \Cref{lem:true_assignment_noisy}, for all clusters $C,C' \in \bigcup_{i=1}^s \scrC_s$, if $\labell(C) = \labell(C')$, then $\labst(C) = \labst(C')$. Set $\pi$ to be the correct permutation thats equivalence classes under $\labell$ to those under $\labst$.
\end{proof}

\begin{definition}[Mistake Term] We say a function $\Mistake(\cdot,\cdot): \N \times (0,1) \to \reals_{\ge 0}$ is an \emph{valid mistake term} if, with probability $1-\delta$, for all $s$ and all $C \in \scrC_s$,
\begin{align*}
\frac{1}{|C|}\sum_{(x,y) \in C} \I\{\gst(x) \ne \labst(C)\} = \frac{1}{|C|}\sum_{(x,y) \in C} \I\{\gst(x) \ne \pi_s \circ \labell(C)\} \le \Mistake(|C|,\delta).
\end{align*}
\end{definition}


==> body/noisy_reg.tex <==
%!TEX root = ../max_scratch.tex


\newcommand{\Exp}{\E}
\newcommand{\Zab}{Z_{a,b}}
\newcommand{\Zbarab}{\bar{Z}_{a,b}}
\newcommand{\Vab}{V_{a,b}}
\newcommand{\Vbarab}{V_{a,b}}
\newcommand{\Prppre}{\Pr_{\barbx = \barbxpre+\barbw}}

\newcommand{\Exppre}{\Exp_{\barbx = \barbxpre+\barbw}}
\newcommand{\barbxpre}{\bar{\bx}_{\mathrm{cln}}}
\newcommand{\bxpre}{\bar{\bx}_{\mathrm{cln}}}

\newcommand{\Zbar}{\bar{Z}}
\newcommand{\bvo}{\bv_{\mathrm{o}}}
\newcommand{\philow}{\phi_{\mathrm{lo}}}
\newcommand{\phimu}{\phi_{\mu}}
\newcommand{\phipz}{\phi_{\mathrm{pz}}}
Let 
\begin{align*}
\Zab(\barbx):= \I\{\gst(\barbx) = a, \ghat(\barbx) = b\}
\end{align*}
We define
\begin{align*}
\Zbarab(\barbxpre) := \E_{\barbw}[Z_{a,b}(\barbx+\barbw)]
\end{align*}
We also compute
\begin{align*}
\Vab(\barbxpre;\barbv) = \Exppre[\langle \barbx, \barbv \rangle^2 \mid Z_{a,b}(\barbx) =1]
\end{align*}
Our goal is to show that there is a function $\psi: \R_{\ge 0} \to \R_{\ge 0}$ such that
\begin{align*}
\Vbarab(\barbxpre;\barbv) \ge \|\barbv\|^2 \psi(\Zbarab(\barbxpre)). 
\end{align*}
\newcommand{\sfp}{\mathsf{p}}
\newcommand{\bdelta}{\boldsymbol{\delta}}
\newcommand{\Var}{\mathbb{V}}
\begin{definition} We define
\begin{align*}
\philow(p,\bdelta) &:= \inf_{\cW \subset \R^d}\{\Var[\langle \bdelta, \bw \rangle \mid \bw \in \cW] : \Pr[\bw \in \cW] = p\} \wedge 1\\
\phimu(p,\bdelta) &:= \sup_{\cW \subset \R^d}\{\langle \bdelta, \Exp[\bw \mid \cW]\rangle^2 : \Pr[\bw \in \cW] = p\}\\
\phipz(p,\bdelta) &:= \sup_{\cW \subset \R^d}\{\Exp[\langle \bdelta, \bw \rangle^4 \mid \bw \in \cW] : \Pr[\bw \in \cW] = p\}^{1/2}\\
\sigma(p,B)^2 &:= \inf_{\bdelta \in\sphere{d},p' \ge p}\frac{\philow(p',\bdelta)}{ \phimu(p',\bdelta) + B^2}\\
\sfp(p,B) &:= \inf_{\bdelta \in\sphere{d},p' \ge p}\left(\frac{\philow(p',\bdelta)}{ (\phimu(p',\bdelta) + B^2)(\phimu(p',\bdelta) + B^2)}\right)^2.\\
\end{align*}
\end{definition}

\begin{lemma}\label{lem:small_bal} There exist universal constants $c_0,c_1$ such that, for any $\barbv \in \cS^d$ with $\bv \ne 0 $ and for any $p \le \Prppre[\barbx \in \cX]$ 
\begin{align*}
\Prppre\left[\langle \barbx, \barbv \rangle^2 \ge c_0 \sigma(p,B)^2 \mid \barbx \in \cX\right] \ge c_1 \sfp(p,B),
\end{align*}
\end{lemma}




\subsection{Proofs}

\begin{lemma}\label{lem:var_lb} Suppose that $B \|\barbx\| \ge 1$, let $\cX \subset \R^{d+1}$, and set $p = \Prppre[\barbx \in \cX]$. Then, for any $\barbv \in \cS^d$ with $\bv \ne 0 $ 
\begin{align*}
\Exppre[\langle \barbx, \barbv \rangle^2 \mid \barbx \in \cX] &\ge \frac{\philow(p,\bdelta) }{2 + 12(\philow(p) + \phimu(p,\bdelta) + B^2  )}, \\
&\gtrsim \frac{\philow(p,\bdelta)}{ \phimu(p,\bdelta) + B^2}, \quad \bdelta = \bv/\|\bv\|.
\end{align*}
\end{lemma}

\begin{lemma}
\label{lem:quad_lb} Under the set up of \Cref{lem:var_lb},
\begin{align*}
\Exppre[\langle \barbx, \barbv \rangle^4 \mid \bx \in \cX] &\le 27\|\barbv\|^4(1+B^4 + \phipz(p,\bdelta)^2) \\
&\lesssim (B^2 + \phipz(p,\bdelta))^2 
\end{align*}
\mscomment{fix $\phipz$ exponent}
\end{lemma}

\begin{proof}[Proof of \Cref{lem:small_bal}] \mscomment{Handle the $\bv = 0$ case. } Let $\sigma^2 := \Exppre[\langle \barbx, \barbv \rangle^2 \mid \barbx \in \cX]$. By the Paley-Zygmud inequality and \Cref{lem:quad_lb,lem:var_lb},
\begin{align*}
\Pr\left[\langle \barbx, \barbv \rangle^2 \ge \frac{\sigma^2}{2} \mid \barbx \in \cX\right] &\ge \frac{\sigma^4}{4\Exppre[\langle \barbx, \barbv \rangle^4 \mid \bx \in \cX]}\\
&\gtrsim (\frac{\philow(p,\bdelta)}{ \phimu(p,\bdelta) + B^2})^2 \cdot (\frac{1}{B^2 + \phipz(p,\bdelta)})^2\\
&\gtrsim \left(\frac{\philow(p,\bdelta)}{ (\phimu(p,\bdelta) + B^2)(\phimu(p,\bdelta) + B^2)}\right)^2.
\end{align*}
\end{proof}
\begin{proof}[Proof of \Cref{lem:var_lb}] 
	We may assume that $\bv \ne 0$, for otherwise  $\barbv$ is supported on its last entry, and the result can be checked directly. Set $\bdelta := \bv/\|\bv\|$.

	Fix $\barbxpre$, define $\barbmu := \Exppre[\barbw]$, so that $\Exppre[\barbx] = \barbxpre + \barbmu$, and let $\cW := \{\bw: \barbx \in \cX\}$. Further, set $p:=\Prppre[\barbx \in \cX] = \Pr[\bw \in \cW]$.
	\begin{align*}
	&\Exppre[\langle \barbx, \barbv \rangle^2 \mid Z_{a,b}(\barbx) =1]\\
	&\ge \Exppre[\langle \barbx - (\barbxpre + \barbmu), \barbv \rangle^2 \mid Z_{a,b}(\barbx) =1]\\
	&= \Exppre[\langle \barbw - \barbmu, \barbv \rangle^2 \mid Z_{a,b}(\barbx) =1]\\
	&= \underbrace{\Exppre[\langle \bw - \bmu, \bv \rangle^2 \mid Z_{a,b}(\barbx) =1]}_{=\tilde V\cdot \|\bv\|^2}\\
	&= \Exppre[\langle \bw - \bmu, \bv \rangle^2 \mid \bw \in \cW]\\
	&= \|\bv\|^2 \philow(p,\bdelta).
	\end{align*}
	On the other hand, using $(x+y)^2 \ge x^2/2 - y^2$
	\begin{align*}
	\Vbarab(\barbxpre;\barbv) &= \Exppre[\langle \barbx, \barbv \rangle^2 \mid Z_{a,b}(\barbx) =1]\\
	&= \Exppre[(\bvo + \langle \bx, \bv \rangle^)2 \mid Z_{a,b}(\barbx) =1]\\
	&\ge \frac{1}{2}\bvo^2 -  \Exppre[ \langle \bx, \bv \rangle^2 \mid Z_{a,b}(\barbx) =1]\\
	\end{align*}
	Moreover, since $\bx = \bxpre + \bw = \bxpre + \bmu +  \bw - \bmu$, we have
	\begin{align*}
	&\Exppre[ \langle \bx, \bv \rangle^2 \mid Z_{a,b}(\barbx) =1] \\
	&\le 3\Exppre[ \langle \bw - \bmu, \bv \rangle^2 \mid Z_{a,b}(\barbx) =1] + 3 \langle \bxpre, \bv \rangle^2  + 3 \langle \barbmu, \bv \rangle^2 \\
	&\le 3(\tilde{V} + \|\bxpre\|^2 + \phimu(p,\bdelta))\|\bv\|^2\\
	\end{align*}
	Thus,
	\begin{align*}
	\Vbarab(\barbxpre;\barbv) \ge \min\left\{\tilde{V}\|\bv\|^2, \frac{1}{2}\bvo^2 - 3(\tilde{V} + B^2 + \phimu(p,\bdelta))\|\bv\|^2\right\}.
	\end{align*}

	Fix an $\alpha := 12(\tilde{V} + B^2 + \phimu(p,\bdelta))$.
	We consider two cases:
	\begin{itemize}
		\item \textbf{Case 1: } $\bvo^2 \le \alpha\|\bv\|^2$. Then $\|\barbv\|^2 = \|\bv\|^2 + \bvo^2  \le (1+\alpha)\|\bv\|^2$
		\begin{align*}
		\Vbarab(\barbxpre;\barbv) &\ge \tilde{V} \|\bv\|^2  \ge \frac{\tilde{V}}{1+\alpha}\|\barbv\|^2.
		\end{align*}
		\item \textbf{Case 2: } We suppose $\|\bvo\|^2 \ge \alpha\|\bv\|^2$. Then 
		 \begin{align*}
	\Vbarab(\barbxpre;\barbv) &\ge  \frac{1}{2}\bvo^2 - 3(\tilde{V} + B^2 + \phimu(p,\bdelta)) \ge \frac{\bvo^2}{4}.
	\end{align*}
	Since $\|\barbv\|^2 = \|\bv\|^2 + \bvo^2 \le (1+\alpha^{-1})\bvo^2$, so
	\begin{align*}
	\Vbarab(\barbxpre;\barbv) \ge \frac{\|\barbv\|^2}{4(1+\alpha^{-1})}. 
	\end{align*}
	Note that $\frac{1^{-1}}{2}+\frac{\alpha^{-1}}{2} \ge (\frac{1}{2}(1+\alpha))^{-1} = 2(1+\alpha)^{-1}$ by Jensen's inequality, so
	\begin{align*}
	\Vbarab(\barbxpre;\barbv) \ge \frac{\|\barbv\|^2}{16(1+\alpha)^{-1}} = \frac{(1+\alpha)\|\barbv\|^2}{16} \ge \tilde{V}\|\barbv\|^2/2.
	\end{align*}
	\end{itemize}
	Thus,
	\begin{align*}
	\frac{\Vbarab(\barbxpre;\barbv)}{\|\barbv\|^2} &\ge \tilde{V}\min\{\frac{1}{2}, \frac{1}{1+\alpha}\} \ge \frac{\tilde{V}}{2 + \alpha}\\
	&= \frac{\tilde{V}}{2 + 12(\tilde{V} + B^2 + \phimu(p))}\\
	&\ge \frac{\philow(p,\bdelta)}{2 + 12(\philow(p) + B^2 + \phimu(p,\bdelta))}.
	\end{align*}
	where in the last line, we use that $x \mapsto (x/(y+x))$ is increasing for $x,y > 0$. 
	\end{proof}

\begin{proof}[Proof of \Cref{lem:quad_lb}]
\begin{align*}
 &\Exppre[\langle \barbx, \barbv \rangle^4 \mid \barbx \in \cX]\\ &= \Exppre[ (\bvo + \langle \bxpre, \bv \rangle +  \langle \bw, \bv \rangle)^2 + \mid \barbx \in \cX]\\
 &= \Exppre[ (\bvo + \langle \bxpre, \bv \rangle +  \langle \bw, \bv \rangle)^2 + \mid \barbx \in \cX]
\end{align*}
Now, we note that Jensen's inequality gives $(\frac{x+y+z}{3})^4 \le \frac{x^3+y^3+z^3}{3}$, so that $(x+y+z)^4 \le 27(x^4+y^4+z^4)$. Thus,
\begin{align*}
&\Exppre[ (\bvo + \langle \bxpre, \bv \rangle +  \langle \bw, \bv \rangle)^2 + \mid Z_{a,b}(\barbx) =1] \\
&\le 27\Exppre\left[ \bvo^4 + \langle \bxpre, \bv \rangle^4 +  \langle \bw, \bv \rangle^4 + \mid \barbx \in \cX\right]\\
&\le 27\|\barbv\|^4\left((1+B^4 + \Exppre[ \langle \bw, \bdelta \rangle^4 + \mid \barbx \in \cX]\right)\\
&\le 27\|\barbv\|^4(1+B^4 + \phipz(p,\bdelta)),
\end{align*}
since for $\barbxpre$, $\{\barbx \in \cX\}$ is just the envent $\{\bw \in \cW\}$ for some set $\cW$.

\end{proof}


==> body/perceptron_old.tex <==
%!TEX root = ../max_scratch.tex

\section{Perceptron}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\bmsf}[1]{\bm{\mathsf{#1}}}
\newcommand{\bsfx}{\bmsf{x}}
\newcommand{\xbar}{\bar{\mathbf{x}}}
\newcommand{\xhat}{\hat{\mathbf{x}}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\ubar}{\bar{\bu}}
\newcommand{\wbar}{\bar{\bw}}
\newcommand{\spread}{\mathsf{p}_w}
\newcommand{\bdelta}{\boldsymbol{\delta}}
\newcommand{\yst}{y^\star}
\newcommand{\bust}{\bu^\star}
\newcommand{\bustbar}{\bar{\bu}^\star}
\newcommand{\delst}{\bdelta^\star}
\newcommand{\Nerr}{N_{\mathrm{err}}}
\newcommand{\distw}{\cD_{w}}
\newcommand{\mistake}{\mathsf{Mistakes}}

\paragraph{Noise model}. We consider $\bx_i = (\xbar_i,1)$, where $\xbar_i = \xhat_i +\wbar_i$, $\wbar_i \sim \distw$. We let
\begin{align*}
\yst_i := \langle \bust, \bx_i \rangle, \quad \bust = (\bustbar,u_d^\star), \quad \bustbar > 0. 
\end{align*}

\begin{definition}[Anti-Concentration Function] Define the anti-concentration function
\begin{align*}
\spread(\eta;\bdelta):= \sup_{a \in \bbR} \Pr_{\wbar \sim \distw} [\langle \wbar,\bdelta \rangle \in [a,a+\eta] ]
\end{align*}
\end{definition}

\begin{lemma}\label{lem:small_margin} Suppose $\bust = (\bustbar,u_d^\star) \in \sphere{d}$, with $\ubar \ne 0$. Then, for any interval $I_0 \subset \bbR$,
\begin{align*}
\Pr[y_i\cdot\langle \bx_i,\bust \rangle \in I_0 \mid \cF_{i-1}] \le 2\spread(\|\bustbar\|^{-1}|I_0|,\delst).
\end{align*}
In particular,  $\Pr[y_i\cdot\langle \bx_i,\bust \rangle \le \gamma\}  \mid \cF_{i-1}] \le 2\spread(\gamma/\|\bustbar\|,\delst)$.
\end{lemma}

\begin{theorem}\label{thm:general mistake} For any $\gamma \in (0,R)$ with probability at least $1-\delta$, the number of mistakes made by the perceptron  is at most
\begin{align*}
%(8N_1 + 4)\frac{R^2}{\gamma^2} + 8m\spread(\gamma/\|\bustbar\|,\delst)  + 32\log(1/\delta)
\# \text{mistakes} \lesssim \frac{R^2\Nerr}{\gamma^2} + m\spread(\gamma/\|\bustbar\|,\delst) + \log(1/\delta), 
\end{align*}
where we define
\begin{align*}
\Nerr := 1+|\{i:y_i \ne \yst\}| 
\end{align*}
\end{theorem}


\begin{definition}[Tsybakov Smoothing]
We say that $\distw$ is  $(\alpha,\beta)$-Tsybakov at $\bust$ if 
\begin{align*}
\spread(\eta;\delst) \le \beta \eta^{1-\alpha}, \quad \delst := \bust/\|\bust\|. 
\end{align*}
\end{definition}
Note tht if the distribution of $\bw$ has density with respect to the Lebesgue measure with density upper bounded by $\beta$, then $\bw$ is $(0,\beta)$-Tsybakov. 
\begin{corollary}\label{cor:Tsyb} Suppose that $\distw$ is $(\alpha,\beta)$-Tsybakov. Define $\rho := \frac{2}{3-\alpha} \in [\frac{2}{3},1)$. Then, with probability $1-\delta$
\begin{align*}
\# \text{mistakes}  \lesssim (\beta m)^{\rho} \cdot (R^2\Nerr )^{1- \rho} \cdot\|\bustbar\|^{\frac{2-2\alpha}{3-\alpha}} + \log(\ceil{\log m }/\delta). 
\end{align*}
\end{corollary}
\newcommand{\Unif}{\mathrm{Unif}}
\begin{proposition}[Information Theoretic Lower Bound] Consider the setting where $\xbar_t \in [1,1]$, and $\wbar_t \sim \Unif([-\alpha,\alpha])$, where $\alpha \le 1/8$. Then, there exists an agnostic adversary which forces the learner to pay expected regret at least 
\begin{align*}
\mathrm{stuff}
\end{align*}
\end{proposition}
\begin{proof} Define $\xhat_t = 1 - t\alpha$. 
\end{proof}
\mscomment{Note, the union bond over $\ceil{\log m}$ comes from allowing a potentially adaptive adversary. }

\subsection{Proofs}
\begin{theorem} Let $(\bx_i,y_i)_{i=1}^m \in \bbR^d \times \bbR$ be a sequence of labeled exampled with $\|\bx_i\| \le R$. Fix $\bu \in \sphere{d}$, $\gamma > 0$, and define the margin errors
\begin{align*}
d_i := d_i(\bu,\gamma) = \max\{0,\gamma - y_i\cdot\langle \bx_i,\bu \rangle \}
\end{align*}
Then, the number of mistakes make by the online perceptrop is at most
\begin{align*}
\frac{(R+D)^2}{\gamma^2}, \quad D = \sqrt{\sum_{i=1}^m d_i^2}
\end{align*}
\end{theorem}
\begin{corollary}\label{cor:mix_mistakes_error} Fix a $\bu \in \sphere{d},\gamma \in (0,R)$. Let 
\begin{align*}
N_{1} &:= |\{i:\sign(y_i \cdot \langle \bx_i, \bu \rangle) < 0\}|\\
N_{2} &:= |\{0 \le y_i\cdot\langle \bx_i,\bu \rangle \in [0,\gamma]\}|
\end{align*}
Then, the number of mistakes make by the online perceptron is at most
\begin{align*}
(8N_1 + 4)\frac{R^2}{\gamma^2} + 2N_2 
\end{align*}
\end{corollary}
\begin{proof}[Proof of \Cref{cor:mix_mistakes_error}] Let $S_{1}:= \{i:\sign(y_i \cdot \langle \bx_i, \bu \rangle) \ne 1\}$ and $S_2 := \{i:\sign(y_i \cdot \langle \bx_i, \bu \rangle) = 1, \quad y_i\cdot\langle \bx_i,\bu \rangle \le \gamma\}$. Note that $N_1 := |S_1|$ and $N_2 := |S_2|$. Moreover, $S_1 \cap S_2 = \emptyset$, and if $i \notin (S_1 \cup S_2)$, $d_i := \max\{0,\gamma - y_i\cdot\langle \bx_i,\bu \rangle \} = 0$. Hence, 
\begin{align*}
D^2 &= \sum_{i \in S_1} d_i^2 + \sum_{j \in S_2} d_j^2\\
&\le N_1 \max_{i \in S_1} d_i^2 + N_2 d_j^2.
\end{align*}
For $i \in S_1$, $d_i^2 \le (\gamma + |\langle \bx_i,\bu \rangle| )^2 \le (\gamma + R)^2 \le 4R^2$, where we used $\gamma \le R$. For $j \in S_2$, $d_j \in [0,\gamma]$, so $d_j^2 \le \gamma^2$. Thus, $D^2 \le 4R^2N_1 + N_2$. Thus, 
\begin{align*}
\frac{(R+D)^2}{\gamma^2} \le \frac{2R^2 +2 D^2}{\gamma^2} \le (8N_1 + 4)\frac{R^2}{\gamma^2} + 2N_2. 
\end{align*}
\end{proof}
\begin{proof}[Proof of \Cref{lem:small_margin}] Note that the ground truth label $y_i$ may depend on $\bx$. We circumvent this with a union bound. Let $I_0$ be any inverval. 
\begin{align*}
\Pr[\yst_i\cdot\langle \bx_i,\bu \rangle \in I_0] &= \Pr[\langle \wbar_i,\ubar \rangle \in y_i(\langle \xhat, \ubar  \rangle + u_d + I_0) ]\\
&\le \sum_{y \in \{-1,+1\}} \Pr[\langle \wbar_i,\ubar \rangle \in y(\langle \xhat, \ubar  \rangle + u_d + I_0) ]\\
&\le \sum_{y \in \{-1,+1\}}\Pr[\langle \wbar_i,\delst \rangle \in \|\bustbar\|^{-1} y(\langle \xhat, \ubar  \rangle + u_d +I_0 ) ]\\
&\le  2\max_{a\subset \bbR}\Pr[\langle \wbar_i,\delst \rangle \in [a, a+ \|\bustbar\|^{-1} |I_0|] ]\\
&\le  2\spread(\|\bustbar\|^{-1}|I_0|,\delst).
\end{align*}
\end{proof}
\begin{proof}[Proof of \Cref{thm:general mistake}] We apply \Cref{cor:mix_mistakes_error} with $\bu = \bust$. Set
\begin{align*}
N_{1} &:= |\{i:\sign(y_i \cdot \langle \bx_i, \bust \rangle) < 0\}|\\
N_{2} &:= |\{i:\sign(y_i \cdot \langle \bx_i, \bust \rangle) = 1, y_i\cdot\langle \bx_i,\bust \rangle \in [0,\gamma]\}|
\end{align*}
it suffices to bound $N_1$ and $N_2$. Sice $\yst_i \cdot \langle \bx_i, \bust \rangle) \ge 0$, we see that each
\begin{align*}
N_1 = \sum_{i=1}^m Z_i, \quad Z_i := \I\{y_i\cdot\langle \bx_i,\bust \rangle \in [0,\gamma]\}.
\end{align*}
Set $t_{\gamma} := 2\spread(\gamma/\|\bustbar\|,\delst) + 8\log(1/\delta)/m$. By \Cref{lem:small_margin},
\begin{align*}
\Exp[Z_i \mid \cF_{i-1}] \le 2\spread(\gamma/\|\bustbar\|,\delst) \le 2t_{\gamma}
\end{align*}
Hence, by a Chernoff bound 
\begin{align*}
\Pr[N_1 \ge 2mt_{\gamma}] = \Pr[\sum_{i=1}^mZ_i \ge 2mt_{\gamma}] \le \exp(-mt_{\gamma}/8) \le \delta.
\end{align*}
Thus, from \Cref{cor:mix_mistakes_error},
\begin{align*}
(8N_1 + 4)\frac{R^2}{\gamma^2} + 4mt_{\gamma} = (8N_1 + 4)\frac{R^2}{\gamma^2} + 8m\spread(\gamma/\|\bustbar\|,\delst)  + 32\log(1/\delta).
\end{align*}

\end{proof}
\begin{proof}[Proof of \Cref{cor:Tsyb}] Fix any $N \in \N$. Under $(\alpha,\beta)$ Tsybakov smoothing, 
\begin{align}
N\frac{R^2}{\gamma^2} + m\spread(\gamma/\|\bustbar\|,\delst ) \le N\frac{R^2}{\gamma^2} + \beta m(\frac{\gamma}{\|\bustbar\|})^{1-\alpha} \label{eq:balance}
\end{align}
Balance both terms by setting $\gamma_N^{3-\alpha} = \|\bustbar\|^{\alpha-1}NR^2/(\beta m)$. Set $\rho = \frac{2}{3-\alpha}$. Then 
\begin{align*}
(N + 1)\frac{R^2}{\gamma_N^2} &= NR^2\cdot (\|\bustbar\|^{\alpha-1}NR^2/\beta m)^{-\rho}\\
&= (\beta m)^{\rho} (NR^2)^{1- \rho} \cdot \|\bustbar\|^{(1-\alpha)\rho}\\
&= (\beta m)^{\rho} (NR^2)^{1- \rho} \cdot\|\bustbar\|^{\frac{2-2\alpha}{3-\alpha}}\\
\end{align*}
Since $\gamma_N^{3-\alpha}$ balanced the terms in \Cref{eq:balance}, we have
\begin{align}
(N + 1)\frac{R^2}{\gamma_N^2} + m\spread(\gamma_N/\|\bustbar\|,\delst ) \le 2 (\beta m)^{\rho} (NR^2)^{1- \rho} \cdot\|\bustbar\|^{\frac{2-2\alpha}{3-\alpha}} \label{eq:gam_choice}
\end{align}
For $k \in \N$, let $\cE_{k}:= \{2^{k-1} \le \Nerr \le 2^k\}$. Then, $\Pr[\bigcup_{k=1}^{\ceil{\log m}}] = 1$. Moreover, by applying \Cref{thm:general mistake} with $\gamma_{2^k}$ for each $k$, we have with probability $1-\delta$, if $\cE_k$ holds, then  applying \Cref{eq:gam_choice} with $N = 2^k$,
\begin{align*}
\# \text{mistakes} &\lesssim \Nerr\frac{R^2}{\gamma_{2^k}^2} + m\spread(\gamma_{(2^k)}/\|\bustbar\|,\delst) + \log(1/\delta)\\
&\lesssim  (\beta m)^{\rho} ((2^k)R^2)^{1- \rho} \cdot\|\bustbar\|^{\frac{2-2\alpha}{3-\alpha}} + \log(1/\delta)\\
&\lesssim  (\beta m)^{\rho} (\Nerr R^2)^{1- \rho} \cdot\|\bustbar\|^{\frac{2-2\alpha}{3-\alpha}} + \log(1/\delta). 
\end{align*}
since $\Nerr \ge 2^k/2$ on $\cE_k$. Taking a union bound over $k \in [\ceil{\log m}]$, with probability $1-\delta$,
\begin{align*}
\# \text{mistakes}  \lesssim (\beta m)^{\rho} (\Nerr R^2)^{1- \rho} \cdot\|\bustbar\|^{\frac{2-2\alpha}{3-\alpha}} + \log(\ceil{\log m }/\delta). 
\end{align*}
\end{proof}

